By My Eyes: Grounding Multimodal Large Language Models with Sensor Data via Visual Prompting

Large language models (LLMs) have demonstrated exceptional abilities across various domains. However, utilizing LLMs for ubiquitous sensing applications remains challenging as existing text-prompt methods show significant performance degradation when handling long sensor data sequences. We propose a visual prompting approach for sensor data using multimodal LLMs (MLLMs). We design a visual prompt that directs MLLMs to utilize visualized sensor data alongside the target sensory task descriptions. Additionally, we introduce a visualization generator that automates the creation of optimal visualizations tailored to a given sensory task, eliminating the need for prior task-specific knowledge. We evaluated our approach on nine sensory tasks involving four sensing modalities, achieving an average of 10% higher accuracy than text-based prompts and reducing token costs by 15.8 times. Our findings highlight the effectiveness and cost-efficiency of visual prompts with MLLMs for various sensory tasks. The source code is available at https://github.com/diamond264/ByMyEyes.

==> backup/instruction.tex <==
\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl\_latex.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
  \centering
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\"a}|     & {\"a}           \\
    \verb|{\^e}|     & {\^e}           \\
    \verb|{\`i}|     & {\`i}           \\
    \verb|{\.I}|     & {\.I}           \\
    \verb|{\o}|      & {\o}            \\
    \verb|{\'u}|     & {\'u}           \\
    \verb|{\aa}|     & {\aa}           \\\hline
  \end{tabular}
  \begin{tabular}{lc}
    \hline
    \textbf{Command} & \textbf{Output} \\
    \hline
    \verb|{\c c}|    & {\c c}          \\
    \verb|{\u g}|    & {\u g}          \\
    \verb|{\l}|      & {\l}            \\
    \verb|{\~n}|     & {\~n}           \\
    \verb|{\H o}|    & {\H o}          \\
    \verb|{\v r}|    & {\v r}          \\
    \verb|{\ss}|     & {\ss}           \\
    \hline
  \end{tabular}
  \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
  \label{tab:accents}
\end{table}

As much as possible, fonts in figures should conform
to the document fonts. See Figure~\ref{fig:experiments} for an example of a figure and its caption.

Using the \verb|graphicx| package graphics files can be included within figure
environment at an appropriate point within the text.
The \verb|graphicx| package supports various optional arguments to control the
appearance of the figure.
You must include it explicitly in the \LaTeX{} preamble (after the
\verb|\documentclass| declaration and before \verb|\begin{document}|) using
\verb|\usepackage{graphicx}|.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{example-image-golden}
  \caption{A figure with a caption that runs for more than one line.
    Example image is usually available through the \texttt{mwe} package
    without even mentioning it in the preamble.}
  \label{fig:experiments}
\end{figure}

\begin{figure*}[t]
  \includegraphics[width=0.48\linewidth]{example-image-a} \hfill
  \includegraphics[width=0.48\linewidth]{example-image-b}
  \caption {A minimal working example to demonstrate how to place
    two images side-by-side.}
\end{figure*}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation:
\begin{quote}
\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
  \centering
  \begin{tabular}{lll}
    \hline
    \textbf{Output}           & \textbf{natbib command} & \textbf{ACL only command} \\
    \hline
    \citep{Gusfield:97}       & \verb|\citep|           &                           \\
    \citealp{Gusfield:97}     & \verb|\citealp|         &                           \\
    \citet{Gusfield:97}       & \verb|\citet|           &                           \\
    \citeyearpar{Gusfield:97} & \verb|\citeyearpar|     &                           \\
    \citeposs{Gusfield:97}    &                         & \verb|\citeposs|          \\
    \hline
  \end{tabular}
  \caption{\label{citation-guide}
    Citation commands supported by the style file.
    The style is based on the natbib package and supports all natbib citation commands.
    It also supports commands defined in previous ACL style files for compatibility.
  }
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

A possessive citation can be made with the command \verb|\citeposs|.
This is not a standard natbib command, so it is generally not compatible
with other style files.

\subsection{References}

\nocite{Ando2005,andrew2007scalable,rasooli-tetrault-2015}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Equations}

An example equation is shown below:
\begin{equation}
  \label{eq:example}
  A = \pi r^2
\end{equation}

Labels for equation numbers, sections, subsections, figures and tables
are all defined with the \verb|\label{label}| command and cross references
to them are made with the \verb|\ref{label}| command.

This an example cross-reference to Equation~\ref{eq:example}.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgments}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya,
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu,
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan,
NAACL 2017 by Margaret Mitchell,
ACL 2012 by Maggie Li and Michael White,
ACL 2010 by Jing-Shin Chang and Philipp Koehn,
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui,
ACL 2005 by Hwee Tou Ng and Kemal Oflazer,
ACL 2002 by Eugene Charniak and Dekang Lin,
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> backup/motivation.tex <==
Current methods~\cite{liu2023large, jin2023large, zhang2024large} for grounding LLMs with sensor data are categorized into two approaches. 
The first approach utilizes specialized features extracted from sensor data, such as R-R intervals for ECG-based arrhythmia detection~\cite{wagner2020ptb}, to compose prompts for specific tasks~\cite{yu2023zero}.
%First, existing approaches~\cite{} compose prompts using specialized features (e.g., XX) extracted from sensor data for specific tasks.
While this approach effectively handles known sensory tasks, %generalizing feature-based prompting across various tasks poses a challenge.
generating feature-based prompts often requires domain knowledge to identify relevant features, which may not be feasible for non-expert users.
% It often requires extensive domain knowledge to identify relevant features, which may not be feasible for non-expert users.
%This method effectively solves known sensory tasks, such as utilizing average heart rate from ECG for arrhythmia dianogsis~\cite{}. 
% However, generalizing the feature-based prompting across different tasks is challenging because it requires domain knowledge to identify relevant features, making it infeasible for non-expert users. 
The second approach~\cite{kim2024health, xu2024penetrative, liu2023large} incorporates raw sensor data directly into prompts as numeric sequences without data processing.
% Recent studies demonstrate that LLMs can interpret these sequences for applications like time-series forecasting~\cite{} and healthcare analytics~\cite{}.
%sequential data for tasks such as time-series forecasting~\cite{} and healthcare applications~\cite{}. 
However, most of these studies focus on short sequences (e.g., fewer than 100 elements)~\cite{kim2024health, xu2024penetrative} and simple tasks (e.g., binary classification)~\cite{liu2023large}. 
% However, existing studies typically involve short sequences (e.g., less than 100 elements)~\cite{} and controlled environments (e.g., binary classification)~\cite{}. 
Addressing the complexity of real-world sensor data remains underexplored, as sensor data often involve longer sequences and more complex tasks~\cite{wang2019survey}. %In this section, we investigate the challenges of using sensor data as text prompts through empirical studies and analysis. 
In this section, we investigate the challenges of using raw sensory signals as text prompts, particularly focusing on the limitations of handling long numeric sequences through empirical studies and analysis.

==> backup/table_backup.tex <==
\begin{table*}[]
\centering
\caption{In progress.}
\label{tab:eval_ssl}
\small
{\renewcommand{\arraystretch}{1.3}
\begin{tabularx}{\textwidth}{LLCCCYCCCY}
\Xhline{2\arrayrulewidth}

 & & \multicolumn{4}{c}{Raw waveform} & \multicolumn{4}{c}{Visualization Planner} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
 & & \multicolumn{2}{c}{Text-only} & \multicolumn{2}{c}{Text+Visual} & \multicolumn{2}{c}{Text-only} & \multicolumn{2}{c}{Text+Visual} \\
Sensor & Dataset & Acc. & Tokens & Acc. & Tokens & Acc. & Tokens & Acc. & Tokens \\

\Xhline{2\arrayrulewidth}

\multirow{3}{*}{Accel.} & HHAR & \makecell{0.66} & 52910 & \cellcolor{my_blue}\textbf{0.70} & \cellcolor{my_blue}2020 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{26.2}\bm{$\downarrow$}})} & 0.66 & 52910 & \cellcolor{my_blue}0.67 & \cellcolor{my_blue}2020 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{26.2}\bm{$\downarrow$}})} \\
 & UTD-MHAD & 0.10 & 50439 & \cellcolor{my_blue}0.41 & \cellcolor{my_blue}5963 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{8.5}\bm{$\downarrow$}})} & 0.10 & 50439 & \cellcolor{my_blue}\textbf{0.43} & \cellcolor{my_blue}5963 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{8.5}\bm{$\downarrow$}})} \\
 & Swimming & 0.50 & 16586 & \cellcolor{my_blue}\textbf{0.74} & \cellcolor{my_blue}1768 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{9.4}\bm{$\downarrow$}})} & 0.51 & 16586 & \cellcolor{my_blue}0.73 & \cellcolor{my_blue}1768 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{9.4}\bm{$\downarrow$}})} \\
\hline
\multirow{4}{*}{ECG} & PTB-XL (CD) & 0.62 & 15224 & \cellcolor{my_blue}0.60 & \cellcolor{my_blue}943 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{16.1}\bm{$\downarrow$}})} & 0.73 & 3204 & \cellcolor{my_blue}\textbf{0.80} & \cellcolor{my_blue}943 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{3.4}\bm{$\downarrow$}})} \\
 & PTB-XL (MI) & \textbf{0.68} & 15228 & \cellcolor{my_blue}0.58 & \cellcolor{my_blue}943 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{16.2}\bm{$\downarrow$}})} & 0.62 & 2766 & \cellcolor{my_blue}\textbf{0.68} & \cellcolor{my_blue}943 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{2.9}\bm{$\downarrow$}})} \\
 & PTB-XL (HYP) & 0.52 & 15224 & \cellcolor{my_blue}0.53 & \cellcolor{my_blue}943 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{16.1}\bm{$\downarrow$}})} & 0.47 & 2757 & \cellcolor{my_blue}\textbf{0.55} & \cellcolor{my_blue}943 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{2.9}\bm{$\downarrow$}})} \\
 & PTB-XL (STTC) & 0.53 & 15229 & \cellcolor{my_blue}0.53 & \cellcolor{my_blue}946 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{16.1}\bm{$\downarrow$}})} & 0.53 & 3596 & \cellcolor{my_blue}\textbf{0.57} & \cellcolor{my_blue}946 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{3.8}\bm{$\downarrow$}})} \\
\hline
EMG & Gesture & 0.15 & 88647 & \cellcolor{my_blue}\textbf{0.30} & \cellcolor{my_blue}3073 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{28.9}\bm{$\downarrow$}})} & 0.27 & 88655 & \cellcolor{my_blue}\textbf{0.30} & \cellcolor{my_blue}3073 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{28.9}\bm{$\downarrow$}})} \\
\hline
Resp. & WESAD & 0.48 & 60253 & \cellcolor{my_blue}\textbf{0.62} & \cellcolor{my_blue}1211 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{49.8}\bm{$\downarrow$}})} & 0.48 & 60253 & \cellcolor{my_blue}0.61 & \cellcolor{my_blue}1211 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{49.8}\bm{$\downarrow$}})} \\
\Xhline{2\arrayrulewidth}
\multicolumn{2}{c}{\cellcolor{my_green}Average} & \cellcolor{my_green}0.47 & \cellcolor{my_green}36648 & \cellcolor{my_green}0.56 & \cellcolor{my_green}1979 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{18.5}\bm{$\downarrow$}})} & \cellcolor{my_green}0.49 & \cellcolor{my_green}31244 & \cellcolor{my_green}\textbf{0.59} & \cellcolor{my_green}1979 \scalebox{1}{(\textcolor{red}{\bm{$\times$}\textbf{15.8}\bm{$\downarrow$}})} \\

\Xhline{2\arrayrulewidth}
\end{tabularx}}
\end{table*}

\begin{table*}[]
\centering
\caption{In progress.}
\label{tab:eval_ssl}
\smaller[1]
{\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\textwidth}{LCCCCCCCCCC}
\Xhline{2\arrayrulewidth}
\addlinespace[0.1cm] 

 & \multicolumn{3}{c}{Accelerometer} & \multicolumn{4}{c}{ECG} & EMG & Resp & \\
\cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}
\multirow{2}{*}{\shortstack{Visualizatoin\\method}} & \multirow{2}{*}{HHAR} & \multirow{2}{*}{\shortstack{UTD-\\MHAD}} & \multirow{2}{*}{Swim} & \multirow{2}{*}{\shortstack{PTB-XL\\(CD)}} & \multirow{2}{*}{\shortstack{PTB-XL\\(MI)}} & \multirow{2}{*}{\shortstack{PTB-XL\\(HYP)}} & \multirow{2}{*}{\shortstack{PTB-XL\\(STTC)}} & \multirow{2}{*}{Gesture} & \multirow{2}{*}{WESAD} & \multirow{2}{*}{Avg.} \\
& & & & & & & & & & \\

\Xhline{2\arrayrulewidth}

\addlinespace[0.1cm]
Raw waveform & 0.80 & 0.55 & 0.82 & 0.75 & 0.78 & 0.70 & 0.72 & 0.40 & 0.75 & 0.75 \\
Visualization Planner & 0.80 & 0.55 & 0.82 & 0.75 & 0.78 & 0.70 & 0.72 & 0.40 & 0.75 & 0.75 \\

% \addlinespace[0.1cm]
\Xhline{2\arrayrulewidth}
\end{tabularx}}
\end{table*}
